Hardware-assisted Trusted Memory Disaggregation for Secure Far Memory

Memory disaggregation provides efficient memory utilization across network-connected systems. It allows a node to use part of memory in remote nodes in the same cluster. Recent studies have improved RDMA-based memory disaggregation systems, supporting lower latency and higher bandwidth than the prior generation of disaggregated memory. However, the current disaggregated memory systems manage remote memory only at coarse granularity due to the limitation of the access validation mechanism of RDMA. In such systems, to support fine-grained remote page allocation, the trustworthiness of all participating systems needs to be assumed, and thus a security breach in a node can propagate to the entire cluster. From the security perspective, the memory-providing node must protect its memory from memory-requesting nodes. On the other hand, the memory-requesting node requires the confidentiality and integrity protection of its memory contents even if they are stored in remote nodes. To address the weak isolation support in the current system, this study proposes a novel hardware-assisted memory disaggregation system. Based on the security features of FPGA, the logic in each per-node FPGA board provides a secure memory disaggregation engine. With its own networks, a set of FPGA-based engines form a trusted memory disaggregation system, which is isolated from the privileged software of each participating node. The secure memory disaggregation system allows fine-grained memory management in memory-providing nodes, while the access validation is guaranteed with the hardware-hardened mechanism. In addition, the proposed system hides the memory access patterns observable from remote nodes, supporting obliviousness. Our evaluation with FPGA implementation shows that such fine-grained secure disaggregated memory is feasible with comparable performance to the latest software-based techniques.

==> tab_commands.tex <==
\begin{table}[t!]
    \footnotesize
    \centering
    \setlength\extrarowheight{1.5pt}
    \begin{tabular}{L{1.5cm}|L{5.7cm}}
        \toprule
        \multicolumn{1}{c}{\textbf{Command}}
            & \multicolumn{1}{c}{\textbf{Description}}\\ \toprule
        Store & Store a page \\
        Load & Load a page \\
        Invalidate Page & Deallocate page from the corresponding memory tier \\
        Invalidate Area & Deallocate pages in all memory tiers \\ \bottomrule
    \end{tabular}
    \vspace{0.5em}
    \caption{Commands in \tdmem.}
    \label{tab:commands}
    \vspace{-0.5em}
\end{table}

